New binary black hole mergers in the LIGO--Virgo O3a data

We report the detection of ten new binary black hole (BBH) mergers in the publicly released data from the the first half of the third observing run (O3a) of advanced LIGO and advanced Virgo. We identify candidates using an updated version of the IAS search pipeline and compile a catalog of signals that pass a significance threshold of astrophysical probability greater than 0.5 (following the GWTC-2.1 and 3-OGC catalogs). The updated IAS pipeline is sensitive to a larger region of parameter space, applies a template prior that accounts for different search volume as a function of intrinsic parameters, and uses an improved coherent detection statistic that optimally combines the data from the Hanford and Livingston detectors. Among the ten new events, we observe interesting astrophysical scenarios including sources with confidently large effective spin parameters in both the positive and negative directions, high-mass black holes that are difficult to form in stellar collapse models due to (pulsational) pair instability, and low-mass mergers that bridge the gap between neutron stars and the lightest observed black holes. We infer source parameters in the upper and lower black hole mass gaps with both extreme and near-unity mass ratios, and one of the possible neutron star--black hole mergers is well localized for electromagnetic counterpart searches. We detect all of the GWTC-2.1 BBH mergers with coincident data in Hanford and Livingston except for three loud events that get vetoed, which is compatible with the false-positive rate of our veto procedure, and three that fall below the detection threshold. We also return to significance the event GW190909_114149, which was reduced to a sub-threshold trigger after its initial appearance in GWTC-2. This amounts to a total of 42 BBH mergers detected by our pipeline's search of the coincident Hanford--Livingston O3a data.

==> extra_tables.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bgroup
\def\arraystretch{1.25}
\begin{table*}
    \centering
    % \setlength\tabcolsep{1pt}
    \caption{Hanford--Livingston coincident events already reported in the GWTC-2.1 catalog \cite{lvc_o3a_deep_gwtc2_1_update_2021} and the 3-OGC catalog \cite{nitz_o3a_3ogc_catalog_2021} as detected by our pipeline. Three events found by LVC in Hanford--Livingston coincidence were vetoed in our search: GW190521, GW190924\_021846, and GW190403\_051519. The following events are not included in this table because they were detected in Livingston--Virgo or Hanford--Virgo coincidence, or single detector search, all of which we have yet to run: GW190910\_112807, GW190925\_232845, GW190620\_030421, GW190630\_185205, GW190708\_232457, and GW190814. The inverse false alarm rate (IFAR) values in the GWTC-2.1 column were taken from the highest (most recent) version number of each event in the GWOSC catalog (\url{https://www.gw-openscience.org/eventapi/json/GWTC-2.1-confident/}), which corresponds to whichever LVC pipeline achieved the highest astrophysical probability for that event in the GWTC-2.1 analysis. The 3-OGC column was taken from the catalog summary data on the \texttt{GitHub} listed in the publication (\url{https://raw.githubusercontent.com/gwastro/3-ogc/master/3-OGC\_top.txt}).}
    \begin{tabular}{|c|c|cc|ccc|ccc|}%cccc|}
        %\hline
        \hline
        \multirow{2}{*}{Event Name} & \multirow{2}{*}{Bank} & \multirow{2}{*}{$\rho_{\rm H}^2$} & \multirow{2}{*}{$\rho_{\rm L}^2$} & \multicolumn{3}{c|}{$p_{\rm astro}$} & \multicolumn{3}{c|}{IFAR (yr)} \\
        %& \multirow{2}{*}{$m_1 {\scriptstyle( \rm M_\odot)}$} & \multirow{2}{*}{$m_2 {\scriptstyle(\rm M_\odot)}$} & \multirow{2}{*}{$\chi_{\rm eff}$} & \multirow{2}{*}{$z$}
         \cline{5-10}
         & & & & \, IAS \, $|$ & $|$ GWTC-2.1 $|$ & $|$ 3-OGC & \,
         IAS\footnote{The IFARs are computed within each bank\changed{, and we do not include any additional trials factor}.} \, $|$ & $|$ GWTC-2.1 $|$ & $|$ 3-OGC \\
         %& & & & \\
         \hline
         \rowcolor{gray!30} GW190403\_051519 & \texttt{BBH\_4} & $23.1$ & $29.7$ & $--$ & $0.61$ & $--$ & Veto & $0.13$ & $--$ \\
GW190408\_181802 & \texttt{BBH\_3} & $95.4$ & $109.2$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190412\_053044 & \texttt{BBH\_2} & $76.2$ & $245.5$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190413\_052954 & \texttt{BBH\_4} & $26.7$ & $50.5$ & $0.83$ & $0.93$ & $0.99$ & $4.2$ & $1.2$ & $1.4$ \\
\rowcolor{gray!30} GW190413\_134308 & \texttt{BBH\_4} & $30.1$ & $62.3$ & $1.00$ & $0.99$ & $0.99$ & $> 1000$ & $2.9$ & $6.4$ \\
GW190421\_213856 & \texttt{BBH\_4} & $68.0$ & $42.0$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $71.4$ & $> 1000$ \\
\rowcolor{gray!30} GW190426\_190642 & \texttt{BBH\_5} & $24.1$ & $42.7$ & $0.33$ & $0.75$ & $--$ & $0.19$ & $0.24$ & $--$ \\
GW190503\_185404 & \texttt{BBH\_3} & $83.2$ & $57.7$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190512\_180714 & \texttt{BBH\_2} & $39.4$ & $119.4$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190513\_205428 & \texttt{BBH\_3} & $78.0$ & $66.0$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190514\_065416 & \texttt{BBH\_4} & $38.9$ & $31.7$ & $0.98$ & $0.76$ & $0.85$ & $290$ & $0.36$ & $0.19$ \\
GW190517\_055101 & \texttt{BBH\_3} & $48.7$ & $58.5$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $9.1$ & $66.1$ \\
\rowcolor{gray!30} GW190519\_153544 & \texttt{BBH\_4} & $81.6$ & $128.7$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190521\_030229 & \texttt{BBH\_5} & $65.0$ & $129.8$ & $--$ & $1.00$ & $1.00$ & Veto & $769$ & $805$ \\
\rowcolor{gray!30} GW190521\_074359 & \texttt{BBH\_3} & $142.3$ & $431.3$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190527\_092055 & \texttt{BBH\_3} & $27.4$ & $46.9$ & $0.92$ & $0.85$ & $0.93$ & $10.8$ & $4.3$ & $0.37$ \\
\rowcolor{gray!30} GW190602\_175927 & \texttt{BBH\_4} & $41.9$ & $111.6$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $391$ \\
GW190701\_203306 & \texttt{BBH\_2} & $25.1$ & $53.8$ & $0.23$ & $1.00$ & $1.00$ & $0.084$ & $1.8$ & $0.13$ \\
\rowcolor{gray!30} GW190706\_222641 & \texttt{BBH\_4} & $91.3$ & $79.2$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $2.9$ & $> 1000$ \\
GW190707\_093326 & \texttt{BBH\_1} & $63.7$ & $97.5$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190719\_215514 & \texttt{BBH\_3} & $37.0$ & $33.2$ & $0.90$ & $0.92$ & $0.89$ & $8.5$ & $1.6$ & $0.25$ \\
GW190720\_000836 & \texttt{BBH\_1} & $44.7$ & $62.3$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $10.6$ & $559$ \\
\rowcolor{gray!30} GW190725\_174728 & \texttt{BBH\_1} & $31.3$ & $59.1$ & $0.96$ & $0.96$ & $0.91$ & $34.2$ & $2.2$ & $0.41$ \\
GW190727\_060333 & \texttt{BBH\_4} & $76.0$ & $61.3$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190728\_064510 & \texttt{BBH\_1} & $58.4$ & $110.1$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190731\_140936 & \texttt{BBH\_3} & $28.9$ & $39.6$ & $0.76$ & $0.83$ & $0.93$ & $2.1$ & $0.53$ & $0.43$ \\
\rowcolor{gray!30} GW190803\_022701 & \texttt{BBH\_3} & $30.6$ & $43.7$ & $0.94$ & $0.97$ & $0.99$ & $15.7$ & $2.6$ & $2.4$ \\
GW190805\_211137 & \texttt{BBH\_4} & $18.8$ & $54.8$ & $0.81$ & $0.95$ & $--$ & $3.3$ & $1.6$ & $--$ \\
\rowcolor{gray!30} GW190828\_063405 & \texttt{BBH\_3} & $112.6$ & $142.3$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190828\_065509 & \texttt{BBH\_2} & $54.5$ & $53.6$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190915\_235702 & \texttt{BBH\_3} & $92.4$ & $71.1$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $> 1000$ & $> 1000$ \\
GW190916\_200658 & \texttt{BBH\_4} & $27.1$ & $36.5$ & $0.93$ & $0.66$ & $0.88$ & $20.7$ & $< 0.001$ & $0.22$ \\
\rowcolor{gray!30} GW190917\_114629 & \texttt{BBH\_0} & $26.8$ & $40.6$ & $0.35$ & $0.77$ & $--$ & $0.17$ & $1.5$ & $--$ \\
GW190924\_021846 & \texttt{BBH\_1} & $31.9$ & $94.9$ & $--$ & $1.00$ & $1.00$ & Veto & $> 1000$ & $> 1000$ \\
\rowcolor{gray!30} GW190926\_050336 & \texttt{BBH\_3} & $45.3$ & $31.4$ & $0.96$ & $0.54$ & $0.88$ & $25.3$ & $0.91$ & $0.27$ \\
GW190929\_012149 & \texttt{BBH\_5} & $40.2$ & $51.2$ & $1.00$ & $0.87$ & $0.98$ & $> 1000$ & $6.2$ & $3.1$ \\
\rowcolor{gray!30} GW190930\_133541 & \texttt{BBH\_1} & $41.1$ & $55.6$ & $1.00$ & $1.00$ & $1.00$ & $> 1000$ & $55.6$ & $295$ \\
         \hline
         %\hline
    \end{tabular}
    \label{tab:lvc events}
\end{table*}
\egroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









%Maybe I'm not following how your assumptions change the nature of the problem, but I do not agree with this computation. 
%The mean of a chi-squared distribution with $k$ DOF is $k$, and this is in units of squared SNR.

I think we also agree that the worst case scenario of 6 independent and unconstrained DOF is not just unrealistically bad but manifestly incorrect, but just for fun let's work with the comparison of chi2(4) to chi2(10).
Now let's say our trials factor is $10^5$ templates (overestimate) matched every 100 ms for the 100 days ($\lessim 10^7$ s) of coincident data we analyzed, which means we aim for a FAR of roughly 1 in $10^13$. 
%For any number of detectors, the log likelihood (that is, the difference in log likelihood between signal and noise models, or equivalently, the log of the likelihood ratio of signal hypothesis to noise hypothesis) maximized over distance is equal to half the SNR-squared of that same template. This tells us that each additional point in log likelihood is worth 2 chi-squared points.
%A jump in the maximum log likelihood of 7 points therefore corresponds to a gain of roughly 14 points in SNR-squared, which is larger than the difference between the inverse survival function of the chi-squared distributions with 10 and 4 DOF at a FAR of 1 in a million. 

To see this how this translates under the chi2 assumption, try: \\
\texttt{>>> quantile = 1e-13 \\
>>> startDOF, endDOF = 4, 10 \\
>>> snr2barStart = scipy.stats.chi2.isf(quantile, startDOF) \\
>>> snr2barEnd = scipy.stats.chi2.isf(quantile, endDOF) \\
>>> lnLbarShift = (snr2barEnd - snr2barStart) / 2 \\
>>> print(startDOF, "DOF to", endDOF, "DOF for FAR =", quantile) \\
>>> print("requires lnL threshold change =", lnLbarShift)}

 and yet even if we push the FAR all the way to $10^{-12}$ the shift in lnL detection bar when moving from a chi-squared with 4 DOF to one with 10 DOF would be 8 (or 16 chi-squared points). The only event where we make a specific note about possible future improvement from HM/precession is GW190711\_030756, which has $2 \ln \mathcal{L}_{\rm max} - \rho_{\rm H}^2 - \rho_{\rm L}^2 \approx 18$, while for GW190707\_083226 we have an even larger improvement with $2 \ln \mathcal{L}_{\rm max} - \rho_{\rm H}^2 - \rho_{\rm L}^2 \approx 19$. On top of these we have GW190910\_012619 PE with and without precession (same model, but in-plane spins set to 0 in one case) giving an evidence ratio of $e^5$ in favor of precession, and another 4 events where Virgo adds 7 or more chi-squared points (note that the bar from 10 to 12 DOF with worst case Virgo would increase by less than 5 chi-squared points even for a FAR of $10^{-12}$). This set of 8 examples justifies more than a tepid suggestion that future searches with HLV coincidence and HM/precession templates might find some of these detections to be more secure, especially considering that these thresholds are drastic overestimates for a coherently integrated score, so I believe our comment on this topic in the paper is conservative.


%It seems that the computation you are doing is a ratio of standard deviations of the chi-squared distribution (sqrt(2k) for k DOF)

%Thus the change from the effectively 9-D model IMRPhenomD (m1, m2, s1z, s2z, time, distance, polarization, RA, DEC) to the nominally 15-D model IMRPhenomXPHM (adding the 4 in-plane spin components and breaking the 22-only degeneracies that make orbital phase and inclination redundant) would add 6 points to the expected value of SNR-squared in the worst case of independent and unconstrained DOF.

%I am talking about the change in DOF of the signal model, which would go from 5 extrinsic (time, distance, polarization, RA, DEC) and 4 intrinsic (m1, m2, s1z, s2z) to 7 extrinsic and 8 intrinsic when adding the 4 in-plane spin components and breaking the 22-only degeneracies that make orbital phase and inclination redundant. Thus the DOF argument I was making was a comparison between the effectively 9-D likelihood model of IMRPhenomD and the nominally 15-D model of IMRPhenomXPHM.

